Federated Learning-based Collaborative Wideband Spectrum Sensing and Scheduling for UAVs in UTM Systems

In this paper, we propose a data-driven framework for collaborative wideband spectrum sensing and scheduling for networked unmanned aerial vehicles (UAVs), which act as the secondary users (SUs) to opportunistically utilize detected "spectrum holes". Our overall framework consists of three main stages. Firstly, in the model training stage, we explore dataset generation in a multi-cell environment and training a machine learning (ML) model using the federated learning (FL) architecture. Unlike the existing studies on FL for wireless that presume datasets are readily available for training, we propose a novel architecture that directly integrates wireless dataset generation, which involves capturing I/Q samples from over-the-air signals in a multi-cell environment, into the FL training process. Secondly, in the collaborative spectrum inference stage, we propose a collaborative spectrum fusion strategy that is compatible with the unmanned aircraft system traffic management (UTM) ecosystem. Finally, in the spectrum scheduling stage, we leverage reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes to the secondary users. To evaluate the proposed methods, we establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework to generate large spectrum datasets that could be used for developing ML/AI-based spectrum management solutions for aerial devices.

==> abstract.tex <==
    In this paper, we propose a data-driven framework for collaborative wideband spectrum sensing and scheduling for networked unmanned aerial vehicles (UAVs), which act as the secondary users (SUs) to opportunistically utilize detected ``spectrum holes''. Our overall framework consists of three main stages. Firstly, in the \emph{model training} stage, we explore dataset generation in a multi-cell environment and training a machine learning (ML) model using the federated learning (FL) architecture. Unlike the existing studies on FL for wireless that presume datasets are readily available for training, we propose a novel architecture that directly integrates wireless dataset generation, which involves capturing I/Q samples from over-the-air signals in a multi-cell environment, into the FL training process. To this purpose, we propose a multi-label classification problem for wideband spectrum sensing to detect multiple spectrum holes simultaneously based on the I/Q samples collected locally by the UAVs. In the traditional FL that employ FedAvg as the aggregating method, each UAV is assigned an equal weight during model aggregation. However, due to the disparities in channel conditions in a multi-cell environment, the FedAvg approach may not generalize effectively for all the UAV locations. To address this issue, we propose a proportional weighted federated averaging method (pwFedAvg) in which the aggregating weights incorporate wireless channel conditions and received signal powers at each individual UAV. As such, the proposed method integrates the intrinsic properties of wireless datasets into the FL algorithm. 
    % to enhance the performance of the UAVs that exhibit better performance,  
    Secondly, in the \emph{collaborative spectrum inference} stage, we propose a collaborative spectrum fusion strategy that is compatible with the unmanned aircraft system traffic management (UTM) ecosystem.
    In particular, we improve the accuracy of spectrum sensing results by combining the individual multi-label classification results from the individual UAVs at a central server. Finally, in the \emph{spectrum scheduling} stage, we leverage reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes to the secondary users. To evaluate the proposed methods, we establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used for developing ML/AI-based spectrum management solutions for aerial devices.
\\
\\
\\








% In this paper, we propose a data-driven framework for collaborative wideband spectrum sensing and scheduling using federated learning (FL) for networked unmanned aerial vehicles (UAVs), which act as the secondary users (SUs) to opportunistically utilize detected spectrum holes. Existing research on FL for wireless commonly presume that the dataset is readily available at the clients. On the contrary, the wireless datasets, which involve capturing I/Q samples from over-the-air signals in a multi-cell environment, differ significantly from these assumptions. To address this challenge and better understand the influence of wireless datasets on the FL training process, our approach integrates dataset generation directly into the FL training process. To this end, we propose a multi-label classification problem for wideband spectrum sensing to detect spectrum holes based on the I/Q samples collected locally by the UAVs. In the FL setting, each UAV trains a machine learning learning (ML) model locally without exchanging the dataset to the FL server. Instead, they exchange the local model gradients to the FL server that aggregates them to form a global model. In traditional FL that employ FedAvg as aggregating method, each UAV is assigned equal weight during model aggregation. However, due to the disparities in channel conditions in a multi-cell environment, the FL model may not generalize effectively for all the UAV locations when employing FedAvg at the FL server. To this purpose, we propose a proportional weighted federated averaging method (pwFedAvg), enhance the performance of the UAVs that exhibit better performance, where the aggregating weights are calculated proportionally to the received signal power at the individual UAVs. In the deployment stage, we propose collaborative spectrum inference to enhance the accuracy of the spectrum sensing results. To this end, the spectrum hole predictions from the multi-class classification by each individual UAV are fused at a server in the unmanned aircraft system traffic management (UTM) ecosystem. In the spectrum scheduling phase, we leverage reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes to the secondary users (i.e., UAVs). To evaluate the proposed methods, we establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used for developing ML/AI-based spectrum management solutions for aerial devices.
% \\
% \\
% \\





%% Old abstract.
%Too much emphasised on FL but the FL results with pwFedAvg are not that much convincing. Instead, our main contribution is the collaborative study/inference. Even though FL didn't improve much we are not loosing much performance from the more robust CL/LL cases. FL + Spectrum fusion is very cost effective and security preserving without loosing performance compared to CL/LL. This should be our motivation and story line. %%


% In this paper, we propose a
% data-driven framework for wideband spectrum sensing using federated learning (FL) for networked unmanned aerial vehicles (UAVs), which act as the secondary users to opportunistically utilize detected spectrum holes.
% Existing research on FL for wireless commonly assumes the complexities of the wireless channel between clients and the FL server while presuming that the dataset is readily available at the clients. However, the wireless datasets, which involve capturing I/Q samples from over-the-air signals in a multi-cell environment, differ significantly from these assumptions. This disparity highlights the necessity for novel approaches to dataset generation and training within FL frameworks tailored to the unique characteristics of such datasets. To address this challenge and better understand the influence of wireless datasets on the FL training process, our approach integrates dataset generation directly into the FL training process. This integration allows us to adapt the training process to the specific nuances of wireless environments, thus enhancing the effectiveness of FL for wideband spectrum sensing in networked UAV systems.
% To this end, we propose a multi-label classification problem for wideband spectrum sensing to detect spectrum holes based on the I/Q samples collected locally by several UAVs in a multi-cell environment. 
% % Each UAV then trains their respective local model by utilizing the locally collected datasets and transmit their model weights to the central server responsible of training a global model. The central server then aggregates the local model weights and transmits the global model weights back to the UAVs to update their local models.
% However, we observed that the traditional federated average (FedAvg) at the central server failed to generalize effectively across all UAV locations. To enhance the performance of the UAVs that exhibit better performance, we propose a proportional weighted federated averaging method (pwFedAvg), where the weights are calculated proportionally to the received power at the UAVs. pwFedAvg penalizes the models  that under perform while enhancing the weights of models that predict spectrum holes more accurately. Our simulation results demonstrate that pwFedAvg yields improved spectrum hole prediction results than the traditional FedAvg for under performing locations. Additionally, we also address collaborative spectrum inference and scheduling for the requesting UAVs by leveraging reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes. To evaluate the proposed methods, we establish a comprehensive emulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the channel usage of primary users in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used to further develop ML/AI-based spectrum management solutions for aerial devices. 


% However, instead of using the traditional federated average (FedAvg) at the central server we propose a proportional weighted federated averaging method (pwFedAvg) and the weights are computed proportionally to the received power at the UAVs. Our simulation results demonstrate that pwFedAvg not only converges faster than the vanilla FedAvg but also yields improved spectrum hole prediction results. Additionally, we also address collaborative spectrum inference and scheduling for the requesting UAVs by leveraging reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes.  To evaluate the proposed methods, we establish a comprehensive emulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the channel usage of primary users in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used to develop ML/AI-based spectrum management solutions for aerial devices. 







% In this paper, we introduce a data-driven framework for wideband spectrum sensing utilizing federated learning (FL) within a networked unmanned aerial vehicle (UAV) system, where UAVs serve as secondary users to exploit detected spectrum gaps opportunistically.

% Existing research on FL for wireless commonly assumes the complexities of the wireless channel between clients and the FL server, presuming that the dataset is readily available at the clients. However, wireless datasets, involving the capture of I/Q samples from over-the-air signals in a multi-cell environment, significantly differ from these assumptions. This discrepancy underscores the need for novel approaches to dataset generation and training within FL frameworks tailored to the unique characteristics of such datasets. To address this challenge and gain insight into the influence of wireless datasets on the FL training process, we integrate dataset generation directly into the FL training process. This integration enables us to adapt the training process to the specific nuances of wireless environments, enhancing the effectiveness of FL for wideband spectrum sensing in networked UAV systems.

% We propose a multi-label classification problem for wideband spectrum sensing to detect spectrum holes based on locally collected I/Q samples by multiple UAVs in a multi-cell environment. Each UAV then trains its respective local model using locally collected datasets and transmits their model weights to the central server responsible for training a global model. Instead of using the traditional federated average (FedAvg) at the central server, we propose a weighted federated averaging method (W-FedAvg), where the weights are computed proportionally to the received power at the UAVs. Our simulation results demonstrate that W-FedAvg not only converges faster than vanilla FedAvg but also yields improved spectrum hole prediction results. Additionally, we address spectrum scheduling for the requesting UAVs by leveraging reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes.

% To evaluate the proposed methods, we establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using the MATLAB LTE toolbox by incorporating base station (BS) locations in a chosen area of interest, performing ray-tracing, and emulating the primary users' channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework for generating large spectrum datasets that could be used for developing ML/AI-based spectrum management solutions for aerial devices.







% Existing research on FL for wireless commonly considers the complexities of the wireless channel between clients and the FL server, presuming that the dataset is readily available at the clients. However, the wireless datasets that involve capturing I/Q samples from over-the-air signal in a multi-cell environment differ significantly from the previously assumed datasets. This disparity underscores the need for novel approaches to dataset generation and training within FL frameworks tailored to the unique characteristics of such datasets. To understand the influence of the wireless datasets on the FL training process, our approach in this work integrates dataset generation directly into the FL training process. To this end, we propose a multi-label classification problem for wideband spectrum sensing to detect spectrum holes based on the I/Q samples collected locally by several UAVs in a multi cell environment.   
% Each UAV then trains their respective local model by utilizing the locally collected datasets and transmit their model weights to the central server responsible of training a global model. The central server then aggregates the local model weights and transmits the global model weights back to the UAVs to update their local models. However, instead of using the traditional federated average (FedAvg) at the central server we propose a weighted federated averaging method (W-FedAvg) and the weights are computed proportionally to the received power at the UAVs. Our simulation results demonstrate that W-FedAvg not only converges faster than the vanilla FedAvg but also yields improved spectrum hole prediction results. Additionally, we also address spectrum scheduling for the requesting UAVs by leveraging reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes.  To evaluate the proposed methods, we establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used for developing ML/AI-based spectrum management solutions for aerial devices.
















% The wideband spectrum sensing involves a training phase and deployment phase. For the training phase, we employ FL, where each UAV is trained on the I/Q samples,  train their respective local models and transmit the model weights to the central server. The central server then aggregates the local model weights and transmits the global model weights back to the UAVs to update their local models.   In the deployment phase, each UAV predicts the spectrum holes based on the collected I/Q samples. To enhance the accuracy of the spectrum sensing module, the outputs from the multi-label classification by each individual UAV are fused at a server in the unmanned aircraft system traffic management (UTM) ecosystem. In the spectrum scheduling phase, we leverage reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes to the secondary users (i.e., UAVs). To evaluate the proposed methods, we establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used for developing ML/AI-based spectrum management solutions for aerial devices.














% Due to their numerous potential applications, unmanned aerial vehicles (UAVs) have recently attracted a lot of attention. 
% Generally, unlicensed spectrum bands are used for the majority of unmanned aerial vehicle (UAV) communications. 
% To enable advanced use-cases for unmanned aerial vehicles (UAVs), cellular networks provide significant coverage for the safe and reliable operation in beyond visual line-of-sight (BVLOS) scenarios. 
% In this paper, we propose a
% data-driven framework for collaborative wideband spectrum sensing and
% scheduling for networked unmanned aerial vehicles (UAVs), which act as the secondary users to opportunistically utilize detected spectrum holes. To this end, we propose a multi-label classification problem for wideband spectrum sensing to detect vacant spectrum spots based on collected I/Q samples. The wideband spectrum sensing involves a training phase and deployment phase. For the training phase, we employ federated learning, where each UAV is trained on the I/Q samples that are collected locally, train their respective local models and transmit the model weights to the central server. The central server then aggregates the local model weights and transmits the global model weights back to the UAVs to update their local models. In the deployment phase, each UAV predicts the spectrum holes based on the collected I/Q samples. To enhance the accuracy of the spectrum sensing module, the outputs from the multi-label classification by each individual UAV are fused at a server in the unmanned aircraft system traffic management (UTM) ecosystem. In the spectrum scheduling phase, we leverage reinforcement learning (RL) solutions to dynamically allocate the detected spectrum holes to the secondary users (i.e., UAVs). To evaluate the proposed methods, we establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station~(BS) locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used for developing ML/AI-based spectrum management solutions for aerial devices.  

% the server will allocate them to the requesting UAV by using reinforcement learning (RL) based approach. 

 % Furthermore, the dataset generation is very flexible and scalable that allow other researchers to quickly configure the setup and obtain their own datasets. We then Furthermore, we propose an open framework for collaborative spectrum sensing and access for UAS.

% However, since UAV applications have not been allocated a specific frequency spectrum, most of the current UAV applications are operating in the unlicensed spectrum. On the other hand, efforts are being made to incorporate UAS into cellular networks to reuse the existing installed infrastructure and the frequency spectrum. 
% However, it is inevitable that wireless networks will become congested due to the quick expansion of applications and the data requirements for UAV applications. In such scenarios, spectrum sharing plays a vital role where the secondary users (SUs) opportunistically use the under utilized spectrum resources of the primary users (PUs) by quickly sensing the spectrum. However, to the best of our knowledge, there is no existing open dataset for exploring machine learning (ML) solutions for spectrum sensing and sharing for UAS applications. 



% However, due to the rapid growth of applications and data demands for UAV applications, it is inevitable that  wireless networks will be saturated.

% For safe operations of multiple UAVs under beyond visual line-of-sight (BVLOS) conditions, the NASA and FAA are in the process of defining the Unmanned Aircraft System Traffic Management (UTM) system.





% n this context, few studies exist that analyze the cellular coverage for UAVs, a few analyze the interference caused by UAVs on the cellular users, and a few studies exist on the saturation analysis for providing on-demand services using UAVs. There exist a different set of studies that provide services to UAV applications in unlicensed band. Due to rapid growth of applications and data demands for UAV applications, it is inevitable that the wireless networks will be saturated. In such scenarios, spectrum sharing plays a vital role. However, to the best of our knowledge, there is no existing open dataset for exploring machine learning (ML) solutions for spectrum sensing for UAVs to explore ML based solutions. To this very purpose, we generate a large synthetic dataset by incorporating the primary channel usage characteristics,






% Cellular networks due to their ubiquitous coverage can offer remote control and payload communication for UAV links for use cases that operate in beyond visual line of sight (BVLOS) conditions

% Ideally, we would like to allocate separate frequency band for each application. However, it is not always feasible to allocate individual spectrum portions for each and every application for many practical reasons. Unmanned aerial vehicles (UAVs) are one such application. UAV wireless communications are not assigned any particular frequency  band. Hence, the commercial UAVs in current day are using the ISM band.  Spectrum sharing allows the secondary users (SUs) to co-exist along with the primary users (PUs) and use the frequency channels opportunistically. In such a dynamic environment, effectively finding out the vacant spectrum spots,a.k.a, spectrum holes is very critical. In this work, we propose a integrated framework for a collaborative UAV spectrum sensing and sharing model that use deep neural network (DNN) to predict the vacant spectrum holes and  reinforcement learning for allocating the spectrum resources. 

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
    \centering
 \includegraphics[width=.8\linewidth]{simplifiedUTM_v2.jpg}
  \caption{Unmanned Aircraft System Traffic Management (UTM) architecture showing the separation between Federal Aviation Administration (FAA) and industry developments; Flight Information Management System (FIMS).}
  \label{fig:utmmodel}
\end{figure}
Unmanned aerial vehicles (UAVs) have attracted significant interest from communications and networking, robotics, and control societies for exploring novel applications such as on-demand connectivity, search-and-rescue operations, situational awareness, to name a few~\cite{menouar2017uav}. As of April 2024, there were roughly 800,000 registered UAVs in the US alone, positioning UAVs as one of the fastest-growing sectors in the aviation industry~\cite{dronenumbers}. Traditionally, UAVs that are used for recreational purposes are operated under visual line of sight (VLOS) conditions. However, real-world and commercial deployments will most likely be in the form of beyond visual line-of-sight (BVLOS), which provides easier access to remote or hazardous areas, less human intervention, and reduced cost of operation~\cite{li2019beyond}. For safe operations of multiple UAVs under BVLOS conditions, NASA and FAA are in the process of defining the UTM system~\cite{kopardekar2016unmanned}. Fig.~\ref{fig:utmmodel} shows a simplified form of the UTM architecture, highlighting the separation between FAA and industry development and deployment responsibilities for the necessary infrastructure, services, and entities that interact within the UTM ecosystem. In this work, we mainly focus on the hierarchical structure between multiple operators and the UAS service supplier (USS), which assists multiple operators in meeting UTM operational requirements, ensuring safe and efficient utilization of the airspace.


The concept of operations within the UTM architecture~\cite{kopardekar2016unmanned} highlights the need for spectrum resources to facilitate wireless communications between UAVs,  UAV operators, and the USS network.
Existing terrestrial mobile networks (for example, 4G LTE and the upcoming 5G-and-beyond) provide significant wireless coverage with relatively low latency, high throughput, and low cost, making the cellular network a good candidate for the operation of UAVs in BVLOS scenarios~\cite{abdalla2021communications}. However, the proliferation of new wireless services and the demand for higher cellular data rates have significantly exacerbated the spectrum crunch that cellular providers are already experiencing. 
Therefore, it is essential to develop dynamic spectrum sensing, inference, and sharing solutions for UAV operations in existing licensed and unlicensed spectrum to enable advanced aerial use cases in BVLOS, such as urban air mobility (UAM) and advanced air mobility (AAM)~\cite{rimjha2021urban,ghazikor2023exploring}. 
 % developing dynamic spectrum management services to sense, assign, and monitor spectrum usage within the UTM architecture is essential %\blue{[citation]}.  


% Within the concept of operations of the UTM architecture~\cite{kopardekar2016unmanned}, the need for spectrum resources arises for wireless communications between the UAVs, the UAV operator, and the USS network.
%  One major reason to consider spectrum sharing techniques is due to the temporary nature of UAV flight operations. Unless the nature of wireless communications involved and the number of simultaneous UAV operations in the same area are not overwhelmingly high, we believe that sharing the spectrum of existing licensed and unlicensed technologies would be economical.  




\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{FLsystemmodelplanes.png}
    %
    \caption{Envisioned FL system model in a Multi-cell wireless network with multiple UAVs.}
    \label{fig:FL-sysmodel}
    %\vspace{-5mm}
\end{figure}

% In general, both licensed and unlicensed spectrum can be used for UTM-enabled UAS operations. Unlicensed spectrum is shared among different users, and thus it includes light regulations that make users more prone to interference from other users. In contrast to unlicensed spectrum, licensed spectrum grants exclusive access to the channel and includes regulatory requirements to fulfill. 

There exists a multitude of prior works on spectrum management frameworks for ground users~\cite{ahmad20205g,uvaydov2021deepsense,cui2019multi,li2020deep,nguyen2018deep}. For instance, the authors in~\cite{li2020deep,uvaydov2021deepsense,cui2019multi} propose deep learning-based wideband spectrum sensing to dynamically detect ``spectrum holes''. Furthermore, the authors in~\cite{nguyen2018deep} propose reinforcement learning~(RL) techniques for spectrum sharing, assuming that spectrum sensing results are readily available. While these data-driven spectrum management frameworks for ground users are available, they are not directly applicable for UTM-enabled UAV operations, due to several factors, such as the widely different wireless channel models and the overall system architecture~\cite{uvaydov2021deepsense,nguyen2018deep}. 
In the context of UAV spectrum sharing systems, the authors in~\cite{kakar2017waveform,shang2020spectrum} proposed spatial spectral sensing~(SSS) to develop efficient spectrum sharing policies for UAV communications aimed at improving the overall spectral efficiency~(SE). However, the SSS models do not consider the spectrum usage pattern of users under realistic scenarios (e.g., ignoring the I/Q level samples), and/or they consider only a single primary user (PU) or secondary user (SU). Moreover, the problem of joint multi-channel wideband spectrum sensing and scheduling among several SUs has not been fully investigated. 


In this paper, we propose a unified and data-driven spectrum sensing and scheduling framework to enable UAVs to effectively share the spectrum with existing primary users. 
% The proposed method is compatible with the UTM deployment model. 
To make our development more concrete and grounded, the problem of joint spectrum sensing and sharing is formulated as an energy efficiency (EE) maximization in a wideband multi-UAV network scenario. Then, we transform the EE optimization problem into a Markov Decision Process (MDP) to maximize the overall throughput of the SUs. At the spectrum sensing stage, we note the inherent hierarchical nature of the UTM architecture with USS (shown in Fig.~\ref{fig:utmmodel}) is a good match for federated learning (FL) based spectrum sensing. For spectrum scheduling stage, we develop RL-based solutions to enable non-manual and automated spectrum resource allocation. 

Particular to the spectrum sensing stage, we propose an FL-based cooperative wideband spectrum sensing across multiple UAVs. To this purpose, we develop a multi-label classification framework to identify spectrum holes based on the observed I/Q samples. Each UAV trains their respective local models using the locally collected datasets and transmits the local model parameters to the central server. Furthermore, we propose a novel proportional
weighted federated averaging~(pwFedAvg) method that incorporates the power level received at each UAV into the FL aggregation algorithm, thereby integrating the dataset generation plane with the FL model training plane, as shown in Fig.~\ref{fig:FL-sysmodel}. 
% The central server then aggregates the local model weights according to the pwFedAvg and transmits the global model weights back to the UAVs to update their local models. 
Once the training process is completed, all UAVs have an updated global model that predicts \emph{spectrum holes}. 
To further enhance the accuracy of the individual spectrum inference results, the predicted spectrum holes from the multi-label classification at each UAV are fused at a central server within the UTM ecosystem. In the spectrum scheduling stage, we develop and implement several RL algorithms, including the standard Q-learning methods to dynamically allocate underutilized spectrum sub-channels to multiple UAVs. We further investigate the performance of the ``vanilla'' deep Q-Network (DQN) and its variations, including double DQN (DDQN) and DDQN with soft-update.





% There exists few studies on federated learning for spectrum sensing~\cite{~\cite{chen2021federated, gao2021fedswap,wasilewska2023secure,khalek2023advances,liu2022wireless}} that either consider a single PU or a single SU. Few works on FL for wireless study the effects of noisy transmissions between the clients and the server and their effect of convergence. However, these studies predominantly assume that datasets are already available at the clients and only discuss about the details on model training plane as shown in Fig~\ref{fig:FL-sysmodel}. Moreover they assume standard image datasets like CIFAR-10, MNIST,etc.,. .However, the wireless datasets that are to be collected over a multi-cell environment are very complex and different than those standard datasets. For example, the dataset obtained at one UAV location might undergo different wireless channel and have different received signal power than the other locations.

Furthermore, one of the primary challenges of using machine learning (ML) based methods for spectrum sensing and scheduling approaches is the need for large amounts of training data. The lack of available spectral data in many cases is a significant obstacle, especially for UAV networks that introduce an additional level of complexity for large-scale experimental data collection. To address this gap, we have developed a comprehensive framework for generating spectrum datasets. This framework models LTE waveform generation and propagation channel in any environment of interest, particularly suitable for UTM-enabled UAV applications. Using the generated dataset, we provide a comprehensive set of numerical results to demonstrate the efficacy of the joint FL-based spectrum sensing, spectrum fusion and RL-based dynamic spectrum allocation to multiple UAVs. 
In summary, the main contributions of this paper are as follows:
% \textbf{(i)} we develop a \emph{joint} spectrum sensing and access framework using raw LTE I/Q data, \textbf{(ii)} the spectrum sensing module identifies multiple spectrum holes in a wideband multi-channel setting, \textbf{(iii)} we use RL-based techniques (i.e., DQN and its variations) to allocate the identified spectrum holes to multiple UAVs, and \textbf{(iv)} the developed solution is based on realistic channel modeling between several LTE BSs and UAVs. 
\begin{itemize}
    \item We develop a spectrum management framework based on the envisioned UTM deployment architecture. To this end, we propose a joint spectrum sensing and scheduling problem for collaborative networked UAVs that operate according to the UTM rules. The joint optimization problem integrates the spectrum sensing results into the spectrum scheduling stage for scenarios with multiple secondary users (i.e., UAVs) and primary users. 
    \item For spectrum sensing, we propose an FL-based solution to enable collaborative model training across distributed UAVs.  We propose the pwFedAvg method that integrates the underlying wireless channel conditions into the FL aggregation step. We also provide the convergence analysis results of the proposed pwFedAvg method.  We demonstrate the benefits of collaborative spectrum sensing through a fusion step. For the spectrum scheduling stage, we develop RL-based solutions leveraging DQN-based approaches.
    % , we show that the central server can dynamically adjust the allocation strategy given the underlying spectrum requests.  
    % To the best of our knowledge, this is the first work to explore the possibility of FL at a system level for the UTM system.
    \item  We outline a methodology for generating large amounts of I/Q dataset for UAVs in a wide geographical area, considering the effects in a multi-cell multi-path environment by incorporating the base-station locations and accurately modeling the environment using ray-tracing methods. 
Based on the established framework, we provide a comprehensive set of numerical results to analyze the performance of pwFedAvg compared with the traditional FedAvg approach, as well as with centralized and local learning. Our results demonstrate the efficacy of the pwFedAvg method for collaborative spectrum sensing, without the need to transfer all I/Q samples to one location as in central learning.  


    % \item Incorporate dataset specific conditions into the FL model training by proportionally adjusting the model weights (pwFedAvg). 
\end{itemize}




% Compared with the existing works in this area, the key contributions of this paper are as follows: \textbf{(i)} we develop a \emph{joint} spectrum sensing and access framework using raw LTE I/Q data, \textbf{(ii)} the spectrum sensing module identifies multiple spectrum holes in a wideband multi-channel setting, \textbf{(iii)} we use RL-based techniques (i.e., DQN and its variations) to allocate the identified spectrum holes to multiple UAVs, and \textbf{(iv)} the developed solution is based on realistic channel modeling between several LTE BSs and UAVs. 



% \begin{itemize}
%     \item Propose FL based system for UTM.
%     \item Generate I/Q dataset for UAVs in multi cell
%     \item Incorporate dataset specific conditions into the model training
%     \item propose joint spectrum sensing scheduling
% \end{itemize}
\noindent 
This paper extends our prior work~\cite{chintareddy2023collaborative} in which we did not investigate the feasibility of  model training using FL methods for UAVs. In contrast, this paper mainly focuses on developing FL-based spectrum sensing by incorporating the wireless datasets captured by multiple UAVs into the FL model training plane, as shown in Fig.~\ref{fig:FL-sysmodel}. Furthermore, we have significantly extended our dataset generation by scaling the size of captured I/Q data samples and increasing the number of reflection and diffraction rays, thereby enhancing the fidelity of emulating the propagation environment.  
% we developed a comprehensive framework for spectrum dataset generation, which models LTE waveform generation and propagation in any environment of interest for UTM-enabled UAV applications. Additionally, we also proposed a data-driven model for joint wideband spectrum sensing and scheduling across several UAVs. However, it is worth mentioning that 
The remainder of this paper is organized as follows. In Section~\ref{sec:relworks}, we review related works. In Section~\ref{sec:sysmodel}, we present the overall system model and problem formulation for FL-based wideband spectrum sensing and collaborative spectrum inference and scheduling. In Section~\ref{sec:proposedflsoln}, we discuss the dataset generation model and the model training aspects of FL based solution to incorporate our proposed pwFedAvg method, followed by a discussion of the convergence analysis of pwFedAvg. In Section~\ref{sec:DSARL}, we present dynamic spectrum allocation using RL. Section~\ref{sec:datasetgen} describes our methodology to generate synthetic spectrum dataset followed by our numerical results in Section~\ref{sec:results}. Finally, Section~\ref{sec:conclusion} concludes the paper.  




% \begin{table}
%     \centering
%     \begin{tabular}{|c|c|}
%         \hline
%          \textbf{Notation} & \textbf{Description}\\
%          \hline
%          $k$& UAV index\\
%          \hline
%          $\mathcal{K}$ & Set of UAVs \\
%          \hline
%          $K$& Total number of UAVs \\
%          \hline
%          $m$& sub-channel/ spectrum hole index \\
%          \hline
%          $M$& Max spectrum holes / sub-channels \\
%          \hline
%          $\mathcal{B}$& set of base-stations \\
%          \hline
%          $b$ & basestation index \\
%          \hline
%          $B$& Total number of base-stations\\
%          \hline
%          $n$& used in majority rule $n$-out-of-$K$\\
%          \hline
%          $\bm{\eta}_k(t)$& noise signal\\
%          \hline
%          ${\bm{s}}_{b}(t)$& total transmitted signal from base-station $b$ at $t$\\
%          % \hline
%          % $O(t)$ & O any function ; t represents the continuous time or analog time\\
%          \hline
%           ${\bm{g}}_{k,b}(t)$ & multi-path channel between base-station~$b$ and UAV~$k$\\
%           \hline
%           $\bm{v}_{b,m}(t)$ &  waveform on $m^{th}$ sub-channel of base-station $b$ at time $t$\\
%           \hline
%           ${\bm{r}}_k(t)$ & received signal at UAV $k$ at time $t$\\ \hline
%           $P_k(t)$ & Received power computed from captured signal in ${\bm{r}}_k(t)$ \\
%           \hline 
%            $\sigma_k ^2(t)$ & represents the noise variance at UAV $k$ at time $t$\\ \hline         
%            ~$\bm{\Tilde{R}}_{k}(t)$&  $J$ I/Q samples from ${\bf{r}}_k(t)$\\ \hline
%            ${\bm{h}}_k(t)$& true label vector observed at UAV $k$\\ \hline
%            $\bm{\widehat{h}}_k(t)$& predicted label vector at UAV $k$\\ \hline
%            $\bm{D}_k$& local dataset at UAV $k$\\
%            \hline           \textit{f($\bm{{\omega}}_k$)}& ML mathematical function\\ \hline
%            $\bm{{\omega}}_k$ & ML model weights \\
%            \hline
%            $\bm{z}(t)$ & Fusion vector\\
%            \hline
%            $\mathcal{W}$& System Bandwidth \\
%            \hline
%            ${\nabla L(\bm{\omega}^t)}$ & Gradient of global model \\
%            \hline
%            $\gamma^t$& learning rate of global model \\
%            \hline
%            $\nabla L_{k}(\bm{\omega}_k^t)$& Local gradients \\
%            \hline
%            $y_{k,m}(t)$& UAV $k$ scheduled for transmission on channel $m$\\
%            \hline
%             $U_{km}(t)$ & transmission utility amount of data transmitted\\
%            \hline
%            $c_{km}(t)$ & collision indicator \\
%            \hline
%            $SC_{k,m}(t)$ & the sensing cost\\ 
%            \hline
%            $AC_{k,m}(t)$ & transmission cost or access cost \\
%            \hline
%      \end{tabular}
%     \vspace{2mm}
%     \caption{Notations and variables used and their purpose}
%     \label{tab:notations used}
% \end{table}



  
 % This platform enables modeling federated learning based cooperative spectrum sensing and sharing for wideband multi-UAV network scenarios, and can be used for scalable generation of large spectrum datasets within an area of interest. 

 
 
 % establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used for developing ML/AI-based spectrum management solutions for aerial users.  

% In summary, our main contributions are as follows.
% \begin{itemize}
%     \item
%     \item 
%     \item 
% \end{itemize}




%%% Flow.. 1) Talk about the UAV and UTM in a gist
% Talk abut spectrum sensing and sharing for UAVs 
% Talk about FL for wireless and highlight the differences
% combine FL + spectrum sensing + dataset config
% Write key contributions and conclude the intro




%%%%%% old contents...

% Unmanned aerial vehicles (UAVs) have attracted significant interests from communications and networking, robotics, and control societies for exploring novel applications such as on-demand connectivity, search-and-rescue operations, situational awareness, to name a few~\cite{menouar2017uav}. 
% % The current innovations are mostly based on the assumption of visual line-of-sight (VLOS) between an aerial vehicle and ground control station. While such efforts are essential, 
% In order to truly unleash the potentials of UAVs, real-world and commercial deployments will most likely be in the form of beyond visual line-of-sight (BVLOS) scenarios, which in turn provide easier access to remote or hazardous areas, less human intervention, and reduced cost of operation~\cite{li2019beyond}. 
% % Yet, compared with the visual line-of-sight (VLOS) conditions, BVLOS carries higher safety risks. 
% For safe operations of multiple UAVs under BVLOS conditions, the NASA and FAA are in the process of defining the Unmanned Aircraft System Traffic Management (UTM) systems~\cite{kopardekar2016unmanned}.
% % to enable advanced UAS use-cases. 


% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/FLsystemmodelplanes.png}
%     %
%     \caption{Envisioned FL system model in a Multi-cell wireless network with multiple UAVs.}
%     \label{fig:ds-sysmodel}
%     %\vspace{-5mm}
% \end{figure}

% % In general, both licensed and unlicensed spectrum can be used for UTM-enabled UAS operations. Unlicensed spectrum is shared among different users, and thus it includes light regulations that make users more prone to interference from other users. In contrast to unlicensed spectrum, licensed spectrum grants exclusive access to the channel and includes regulatory requirements to fulfill. 
% Existing terrestrial mobile networks (e.g., 4G LTE and the upcoming 5G-and-beyond) provide significant wireless coverage with relatively low latency, high throughput, and low cost. This, in turn, will make the cellular network a good  candidate for the operation of UAVs in BVLOS scenarios~\cite{abdalla2021communications}. %~\cite{takacs2018drones,wang2018bandwidth,abdalla2021communications}.  
% However, the proliferation of new wireless services and the demand for higher cellular data rates have significantly exacerbated the spectrum crunch that cellular providers are already experiencing. Therefore, developing  dynamic spectrum management services to sense, assign, and monitor spectrum usage within the UTM architecture is of utmost importance in order to enable advanced UAV use cases in BVLOS, such as urban air mobility (UAM) and advanced air mobility (AAM)~\cite{rimjha2021urban}. %\blue{[citation]}.  
% % 4G LTE and the upcoming 5G-and-beyond networks support a variety of capabilities that can be leveraged for UAS applications. 
% % Deployments can be further customized by using network slicing for flexible differentiated QoS in terms of latency, throughput, and reliability \blue{[citation]}. 
% % Several recent works have been focused on evaluating the performance of UAVs in LTE networks~\cite{wang2018bandwidth,abdalla2021communications}. 
% % Thanks to the ubiquitous wireless connectivity of LTE and improved capabilities of 5G networks, mobile networks are capable of supporting the initial deployment of low-altitude UAVs for BVLOS  missions~\cite{takacs2018drones}. 





% % LTE Support for Aerials Vehicles has been included as part of 3GPP Rel-15~\cite{muruganathan2018overview}, suggesting that the existing mobile LTE networks can offer wide-area wireless connectivity to the UAS as well. Additionally, several KPI's are defined in 3GPP release 17 and 18 to include UAVs into the cellular network. For instance, the UL and DL requirements for different UAV applications range from 300 Kbps to 100 Mbps~\cite{3GPPTS22125}. Few applications such as surveillance, delivery using line-of-sight links, video streaming, cellular-assisted UAV communication where an UAV can act as a base-station, demand such high data rates. 


% % Contrary to that, few studies as in~\cite{wang2018bandwidth,abdalla2021communications} has been conducted to evaluate the performance of UAVs in LTE networks. 
% % It is concluded that UAVs supporting high data rate applications such as surveillance, delivery using line-of-sight links, video streaming, etc.,. would eventually saturate the cellular network. 

% % Supporting the safe and reliable operation of UAVs in BVLOS scenarios require two main functionalities: (i) real-time delivery of latency-sensitive command-and-control (C2) signals, and (ii)
% % high-throughput payload data channel. 



% % the existing spectrum demand and the anticipated new UAV applications, we have to consider spectrum sharing for UAVs. 

% There exists a multitude of prior works on spectrum management frameworks for ground users~\cite{zhang20196g,ahmad20205g,uvaydov2021deepsense,cui2019multi,li2020deep,nguyen2018deep}. For instance, the authors in ~\cite{li2020deep,uvaydov2021deepsense,cui2019multi} propose deep learning based wideband spectrum sensing to dynamically detect ``spectrum holes''. Furthermore, several studies leverage reinforcement learning (RL) techniques for spectrum sharing, assuming that the spectrum sensing results are readily available~\cite{nguyen2018deep}. While these data-driven spectrum management frameworks for ground users are available, they are not directly applicable for UTM-enabled UAV operations, due to several factors, such as widely different wireless channel models and the overall system architecture~\cite{uvaydov2021deepsense,nguyen2018deep}. 
% In the context of UAV spectrum systems, the authors in~\cite{kakar2017waveform,shang2020spectrum} have developed efficient spectrum sharing policies for UAV communications to enhance the spectral efficiency (SE). However, the majority of the existing spatial spectral sensing (SSS) models do not consider the spectrum usage pattern of users under realistic scenarios (e.g., ignoring the I/Q level samples), and/or they consider only a single primary user (PU) or secondary user (SU). Moreover, the problem of joint multi-channel wideband spectrum sensing and scheduling among several SU's has not been fully investigated. 

% To address these gaps, in the previous work~\cite{chintareddy2023collaborative}, we proposed a data-driven model for joint wideband spectrum sensing and scheduling across several UAVs, which act as secondary users to opportunistically utilize detected spectrum holes.  Our proposed system model presents a unified framework that is compatible with the UTM deployment models with centralized controlling and monitoring entities (e.g., UAS service suppliers). To make our development more concrete and grounded, the problem of joint spectrum sensing and sharing is formulated as an energy efficiency (EE) maximization in a wideband multi-UAV network scenario. Then, we transform the EE optimization problem into a Markov Decision Process (MDP) to maximize the overall throughput of the SUs. To enable wideband spectrum sensing, we develop a multi-label classification framework to identify spectrum holes based on observed I/Q samples. In this paper, we further extend our study to propose federated learning based cooperative wideband sensing. In this context, wideband spectrum sensing involves a training phase and a deployment phase. In the training phase, we employ federated learning based cooperative wideband spectrum sensing, where each UAV is trained on the I/Q samples that are collected locally by each UAV, train their respective local models and send the model weights to the central server. The central server then aggregates the local model weights and transmits the global model weights back to the UAVs to update their local models. Once the training process is complete, all of the UAVs have an updated global model which predicts the \emph{spectrum holes}. Additionally, we analyze the performance of the ML model in two different configurations, namely, centralized learning, local learning. To further enhance the accuracy of the spectrum sensing module, the predicted spectrum holes from the multi-label classification by each individual UAV are fused at the central server. In the spectrum scheduling phase, we develop and implement several RL algorithms, including the standard Q-learning methods to dynamically allocate underutilized spectrum sub-channels to multiple UAVs. We further investigate the performance of the ``vanilla'' deep Q-Network (DQN) and its variations, including double DQN (DDQN) and DDQN with soft-update. \blue{[New RL here]}.  
 
 
%  Furthermore, one of the primary challenges of using machine learning (ML) methods for spectrum management is the need for large amounts of training data. The lack of available spectral data in many cases is a significant obstacle, especially for UAV networks that introduce additional complexity for large-scale experimental data collection. To address this gap, and evaluate the proposed methods, we develop a comprehensive framework for spectrum dataset generation, which accurately models LTE waveform generation and propagation in any environment of interest for UTM-enabled UAV applications. This platform enables modeling federated learning based cooperative spectrum sensing and sharing for wideband multi-UAV network scenarios, and can be used for scalable generation of large spectrum datasets within an area of interest. 
 
 
 
%  % establish a comprehensive simulation framework that generates a near-realistic synthetic dataset using MATLAB LTE toolbox by incorporating base-station locations in a chosen area of interest, performing ray-tracing, and emulating the primary users channel usage in terms of I/Q samples. This evaluation methodology provides a flexible framework  to generate \emph{large spectrum datasets} that could be used for developing ML/AI-based spectrum management solutions for aerial users.  

% % In summary, our main contributions are as follows.
% % \begin{itemize}
% %     \item
% %     \item 
% %     \item 
% % \end{itemize}
% The rest of this paper is organized as follows. In Section~\ref{sec:motivation}, we provide high level introduction of the UTM architecture and highlight the importance of dynamic spectrum sharing in UTM systems. In Section~\ref{sec:relworks}, we review related works on spectrum sensing and sharing.  In Section~\ref{sec:problem}, we discuss our system model, followed by the problem formulation for joint spectrum sensing and access in Section~\ref{sec:problem2}.  Section~\ref{sec:datasetgen} describes our methodology to generate synthetic spectrum dataset, and Section~\ref{sec:results} includes our numerical results, finally we conclude the paper in Section~\ref{sec:conclusion}.

% \blue{[There is no mention of FL in introduction. Need to incorporate new contents with globecom materials.]} --
% \teal{[Revised, need proofreading]}

















 
 % To the best of our knowledge, this is the first paper that proposes  







% to the best of our knowledge, we are not aware of any data driven model that enable UAV communications for UTM systems. In particular, one of the primary challenges of using machine learning (ML) methods for spectrum sensing is the need for large amounts of training data. The lack of available spectral data in many cases is a significant obstacle for developing such data driven methods especially for UAV communications. Moreover, joint spectrum sensing and access in dynamic UAV environments will make the problem even more challenging.

% To this end we propose a method to generate a large amount of synthetic dataset considering realistic LTE base station deployment using MATLAB. We make use of ray-tracing techniques to accurately model the channel dynamics between the base-station and UAVs. Furthermore, to bridge the gap between spectrum sensing and sharing, we propose an end-to-end framework that integrates ML based spectrum sensing and RL based spectrum sharing methods in a multi-channel multi-UAV dynamic environment. As shown in Fig.~\ref{fig:sysmodel} our proposed system model presents a unified framework that is compatible with the UTM deployment models.

% However, the works so far didn't consider an integrated solution that detects the spectrum holes and allocates spectrum resources to the requesting UAVs. In this paper, we propose a coordinated spectrum sensing and sharing platform for UAVs.








% It is concluded that 50 drones transmitting HD video streams continuously can saturate the theoretical uplink capacity of 500 Mbps in a 4G LTE cell that covers a large rural area. Moreover, if the transmissions use 4k video streaming, the number of UAVs that can be supported in a cell further scales down~\cite{abdalla2021communications}. It is clearly evident that UAVs with higher video resolution will saturate the 4G/5G network.

% As the demand for UAV applications increases, the UAV density increases. Hence, there would be a spectrum scarcity similar to the ground-based communications. In order to cope up with the existing spectrum demand and the anticipated new UAV applications, we have to consider dynamic spectrum sharing for UAVs. Few research exists on the theoretical aspects of the spectrum sharing for UAVs.





% While spectrum sensing plays a vital role in allocating spectrum resources to the SUs, to develop such data driven ML-based models, there exists a demand for datasets that captures the PU channel usage characteristics in such dynamic multi-UAV environments. Moreover, the dataset generation should be flexible and scalable such that more complex characteristics can be simulated. 

% The majority of the existing works are based on simplistic assumptions on the underlying spectrum usage patterns. To fill this gap, we generate a large synthetic LTE waveform dataset, and use raw I/Q samples for spectrum sensing. This resembles the actual hardware operation. Moreover,  most of the prior works consider individual UAVs responsible for spectrum sensing, while our proposed solution considers a network of UAVs. Finally, there are limited works on integrated spectrum sensing and sharing with networked UAVs. As shown in Fig.~\ref{fig:sysmodel} our proposed system model presents a unified framework that is compatible with the UTM deployment models. 







% The rest of this paper is organized as follows. In section \ref{sec:related} we briefly discuss about related works, section \ref{sec:problem} presents the system model and problem formulation. We further discuss about the MDP formulation and show how we can apply RL methods for solving the multi-UAV multi-channel environment. In section~\ref{sec:DSA} we discuss about Q-learning (DDQN), the training setup of the DDQN agent and the algorithm that maximizes the total utility. In Section~\ref{sec:dataset} we describe about our synthetic spectrum dataset generation framework for wideband spectrum sensing. Section~\ref{sec:results} includes our numerical results, and Section \ref{sec:conclusion} concludes the paper.

% %############### New content
% \section{Related Work}
% \label{sec:related}
% {
% As the demand for UAV applications increases, the UAV density increases. Hence, there would be a spectrum scarcity similar to the ground-based communications. In order to cope up with the existing spectrum demand and the anticipated new UAV applications, we have to consider dynamic spectrum sharing for UAVs. Few research exists on the theoretical aspects of the spectrum sharing for UAVs. Authors in ~\cite{shang2020spectrum} investigate the need to design efficient spectrum sharing policies for UAV communications to enhance the spectral efficiency (SE) while simultaneously controlling the interference-to-ground communications. Furthermore they propose spatial spectrum sensing (SSS) for UAV spectrum access and address several open research problems and challenges in applying SSS for UAV networks. }

% % While SSS was based on theoretical stochastic geometry based, to the best of our knowledge we are not aware of any data driven spectrum sensing models for UAV.

% % However, there are several data driven spectrum sensing models proposed for cognitive radio networks (CRN).  Also, the above mentioned works do not consider physical characteristics of a dynamic environment. However, the techniques do not consider dynamic UAV environments.


% On the other hand, spectrum sharing in ground based communications is an active research area where same spectrum is shared among multiple technologies. To this end, there are several data driven spectrum sensing models that take advantage of deep learning methods. Specifically, authors in ~\cite{li2020deep,uvaydov2021deepsense,cui2019multi}, propose deep learning based spectrum sensing where spectrum holes are identified when primary users are not transmitting. Few studies build reinforcement learning (RL) based methods for spectrum sharing assuming the sensing sensing results are readily available~\cite{nguyen2018deep}. 

% While there exists a multitude of existing research on data driven models for ground based communications catering spectrum sensing and sharing, to the best of our knowledge, we are not aware of any data driven model for UAV communications. In particular, one of the primary challenges of using machine learning (ML) methods for spectrum sensing is the need for large amounts of training data. The lack of available spectral data in many cases is a significant obstacle for developing such data driven methods especially for UAV communications. Moreover, joint spectrum sensing and access in dynamic UAV environments will make the problem even more challenging.

% To this end we propose a method to generate a large amount of synthetic dataset considering realistic LTE base station deployment using MATLAB. We make use of ray-tracing techniques to accurately model the channel dynamics between the base-station and UAVs. Furthermore, to bridge the gap between spectrum sensing and sharing, we propose an end-to-end framework that integrates ML based spectrum sensing and RL based spectrum sharing methods in a multi-channel multi-UAV dynamic environment.



% Studies in the context of UAVs proposed are either based on stochastic geometry~\cite{shang2020spectrum} or are only applicable for cooperative communication between UAVs in a swarm network ~\cite{wang2020machine}. 


% Authors in ~\cite{cui2019multi} explore resource allocation strategies for UAVs based on multi agent reinforcement learning (MARL) framework. However, the UAVs are non co-operative and randomly select a channel to transmit.

% However, the works so far didn't consider an integrated solution that detects the spectrum holes and allocates spectrum resources to the requesting UAVs. In this paper, we propose a coordinated spectrum sensing and sharing platform for UAVs.


%###################


% A multitude of prior works have been devoted to develop various spectrum sensing and sharing~\cite{li2020deep,uvaydov2021deepsense, shang2020spectrum} and access policies~\cite{nguyen2018deep,cui2019multi} for different applications, ranging from cognitive networks to UAV networks. However,  the majority of the existing works consider a simplified scenario. In particular,  one of the primary challenges of using machine learning (ML) methods for spectrum sensing and access is the need for large amounts of training data. The lack of available data in many cases is a significant obstacle for these methods. Moreover, joint spectrum sensing and access will make the problem even more challenging.





% The rest of this paper is organized as follows. In Section \ref{sec:background} we provide a brief summary of related works. Section \ref{sec:problem} presents the system model and problem formulation. We further discuss about the MDP formulation and show how we can apply RL methods for solving the multi-UAV multi-channel environment. In section~\ref{sec: DSA} we discuss about Q-learning (DDQN),  the training setup of the DDQN agent and the algorithm that maximizes the total utility. In Section~\ref{sec:dataset} we describe about our synthetic spectrum dataset generation framework for wideband spectrum sensing. Section~\ref{sec:results} includes our numerical results, and Section \ref{sec:conclusion} concludes the paper.


% Notations:
% x:scalar, \textbf{x}:vector, \textbf{X}: Matrix


==> motivation.tex <==
% \section{UTM System Architecture and Motivation}
% \label{sec:motivation}
% \blue{Introduce the need for UTM overall concept of UTM}\\
% \blue{Write two or three paras on UTM in the introduction}\\
% \blue{How FL can be used in UTM}\\
% \blue{Highlight the part of Ray-tracing and I/Q dataset generation}\\
% \blue{Conclude with main contributions}

% \subsection{UTM System Architecture}
% \blue{[Shorten this sub-section... too much information about FAA/UTM.]} -- \teal{[Mostly modified]}






% Majority of the UAV applications are operated in lower altitude airspace~(upto $400$ feet above ground level), commonly referred as uncontrolled class G airspace~\cite{whitley2020faa}. Class G airspace generally lacks the surveillance and communications infrastructure and is identified that the existing Air Traffic Management (ATM) System infrastructure cannot scale cost-effectively with UAV density to provide traditional traffic management services.




% UTM is defined as the manner in which the FAA will support operations for UAS operating in low altitude airspace. UTM utilizes industry’s ability to supply services under the FAA’s regulatory authority where these services do not currently exist. It is a community-based traffic management system, where the Operators and entities providing operation support services are responsible for the coordination, execution, and management of operations, with rules of the road established by FAA. This federated set of services enables cooperative management of operations between UAS Operators, facilitated by third-party support providers through networked information exchanges.
% promote shared situational awareness among Operators.


% The concept of UTM is the FAA's approach to support low-altitude airspace operations for the UAVs. The UTM network leverages the industry's capacity to provide services within the framework of FAA regulations, especially in areas where these services are currently lacking. Hence, UTM is a community-based system where multiple UAV operators and UAV service suppliers (USS) coordinate, execute, and manage operations, with FAA-defined rules. This collaborative networked system not only enables cooperative management of UAV operations but also promote shared situational awareness among multiple operators~\cite{UTMimpl}.






% The FAA still controls the regulatory and operational authority for airspace and
% air traffic operations for the UAVs, however, these operations are not managed by the ATM. Instead, they are organized and coordinated by a group of entities within the UTM system.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/simplifiedUTM_v2.jpg}
%      %\vspace{-5mm}
%     \caption{Simplified UTM architecture showing the sepeartion between FAA and Industry developments.}
%     \label{fig:utmmodel} 
%     \vspace{-6mm}
% \end{figure}


% \begin{figure}[!htb]
% \minipage{0.5\textwidth}
% \centering
%    \includegraphics[width=1.1\linewidth]{figures/simplifiedUTM_v2.jpg}
%     % \caption{KPIs for UAV-assisted wireless services according to 3GPP TS 22.125, V17.1.0 }
%     % \label{fig:KPIWS}
%   % \includegraphics[width=\linewidth]{Figures/s.jpg}
%   \caption{Simplified UTM architecture showing the separation between FAA and Industry developments. }
%   \label{fig:utmmodel}
% \endminipage\hfill
% \vspace{2mm}
% \minipage{0.48\linewidth}
% \centering
%   \includegraphics[width=0.78\linewidth]{figures/sc1.jpg}
%   \caption{Deployment scenario 1}
%   \label{fig:sc1}
%   \vspace{5mm}
%       \includegraphics[width=0.78\linewidth]{figures/sc2.jpg}
%   \caption{Deployment scenario 2}
%   \label{fig:sc2}
% \endminipage
% \end{figure}


 

% The UTM architecture is being developed to orchestrate safe operations in BVLOS conditions on the assumption that the existing cellular technologies and the unlicensed spectrum would be able to support the UTM architecture. \blue{Insert this sentence, Note that, within the concept of operations of the UTM, the need for spectrum resources arise for the wireless communications involved between the UAV, the UAV operator and the USS. }However, with the exponential growth~\cite{dronenumbers}, we expect that the demand for spectrum resources for UAV operations would significantly increase. While it would be certainly beneficial to allocate a chunk of spectrum for UAV operations in the long run, we explore dynamic spectrum sharing options for UAV operations in the existing licensed and unlicensed spectrum. One major reason to consider spectrum sharing techniques is due to the temporary nature of UAV flight operations. Unless the nature of wireless communications involved and the number of simultaneous UAV operations are not overwhelmingly high, we believe that sharing the spectrum of existing licensed and unlicensed technologies would be economical.  \blue{check above para again. My intention here is to undermine the spectrum allocation for UAVs when there are only few flight operations and use our proposed solution, however, down the line when this situation changes and the number of simulataneous UAV operations in a specific area significantly grow, alloting spectrum would be beneficial.}

% The UTM architecture is being developed to orchestrate safe operation of multiple UAVs on the pretext that the existing cellular technologies and the unlicensed spectrum would be able to support BVLOS operations. Within the concept of operations of the UTM architecture, as shown in Fig.~\ref{fig:utmmodel}, the need for spectrum resources arise for the wireless communications involved between the UAV, the UAV operator and the USS network. However, with the exponential growth of UAV applications~\cite{dronenumbers}, we expect that the demand for spectrum resources would significantly increase. While it would be certainly beneficial to allocate a chunk of spectrum dedicated for UAV operations in the long run, we explore dynamic spectrum sharing options for UAV operations in the existing licensed and unlicensed spectrum. One major reason to consider spectrum sharing techniques is due to the temporary nature of UAV flight operations. Unless the nature of wireless communications involved and the number of simultaneous UAV operations in the same area are not overwhelmingly high, we believe that sharing the spectrum of existing licensed and unlicensed technologies would be economical.

% \subsection{Motivation}


%To this end, we demonstrate a data driven FL model as shown in~\ref{fig:trainphase}.




%%%%%% Old content \\\
% \subsection{Motivation}
% Within the concept of operations of the UTM architecture, as shown in Fig.~\ref{fig:utmmodel}, the need for spectrum resources arise for the wireless communications involved between the UAV, the UAV operator and the USS network. However, with the exponential growth of UAV applications~\cite{dronenumbers}, we expect that the demand for spectrum resources would significantly increase. Hence, we explore dynamic spectrum sharing options for UAV operations in the existing licensed and unlicensed spectrum. One major reason to consider spectrum sharing techniques is due to the temporary nature of UAV flight operations. Unless the nature of wireless communications involved and the number of simultaneous UAV operations in the same area are not overwhelmingly high, we believe that sharing the spectrum of existing licensed and unlicensed technologies would be economical.  
% % \blue{check above para again. My intention here is to undermine the spectrum allocation for UAVs when there are only few flight operations and use our proposed solution, however, down the line when this situation changes and the number of simultaneous UAV operations in a specific area significantly grow, allotting spectrum would be beneficial.}


% Furthermore, the inherent hierarchical nature of UTM architecture, shown in Fig.~\ref{fig:utmmodel}, is a good match for federated learning (FL) based spectrum sharing. To this end, we envision two FL scenarios within the UTM architecture. One scenario would be having a FL server at each operator where multiple UAVs connected to the operator act as FL clients, as shown in Fig.~\ref{fig:sc1}. While the other scenario would have a FL server within the USS network that can orchestrate multiple operator and multiple UAVs, as shown in Fig.~\ref{fig:sc2}. To enhance the performance of wideband spectrum sensing, multiple UAVs connected with multiple operators across the USS network can collaborate, thereby defying the need for separate training at each location. 

% Given that the architectural advantage of UTM architecture we propose an FL based cooperative wideband spectrum sensing system that enables UAVs to effectively share the spectrum with existing primary users. To this end, we demonstrate a data driven FL model as shown in~\ref{fig:trainphase}.
%%%%%% Old content ////

% the need for spectrum resources arise for the communication involved between the UAV, the UAV operator and the USS. The 

% \blue{Add about the Operator, USS and entities defined in the block diagram. Next highlight the spectrum I/Q for BVLOS and bring in the contributions including the FL part}


% Figure 3 depicts a notional UTM architecture that
% visually identifies, at a high level, the various actors and components, their contextual relationships, as
% well as high-level functions and information flows. The gray dashed line in Figure 3 represents the
% demarcation between the FAA and industry responsibilities for the infrastructure, services, and entities
% that interact as part of UTM. As shown, UTM comprises a sophisticated relationship between the FAA,
% the Operator, and the various entities providing services and/or demonstrating a demand for services
% within the UTM ecosystem. The illustration highlights a model, which heavily leverages utilization of thirdparty
% entities to support the FAA and the Operator in their respective roles and responsibilities. Sections
% 2.3.1 and 2.3.2 describe elements of this notional architecture.


% to provide traditional air traffic management services, especially as the density of UAV operations increases over time.

% Given the number and type of UAV operations envisioned, it is identified that the existing Air Traffic Management (ATM) System infrastructure cannot scale cost-effectively 
% to support the exponential growth UAS.


% While BVLOS applications have several advantages they pose several safety and security concerns. 



% To address such problems,  for safe operations of multiple UAVs under BVLOS conditions. 


% While the concept of UTM is being developed to support and enable scalable and safe BVLOS UAV operations, it is specifically defined for UAVs operating in lower altitude airspace~(upto 400 feet above ground level), commonly referred as class G airspace~\cite{}


% In early 2020, the FAA published Version 2 of the UTM ConOps, which contained a number of important definitions and settled several policy topics related to UTM. Specifically, the UTM ConOps specified that UTM is for managing drones at altitudes up to 400 feet AGL, which is often referred to as “low altitude airspace” [3, Page 4]. UTM services could exist in controlled airspace, which includes Class B, C, D, or E airspace; or in uncontrolled Class G airspace
% Class G airspace generally lacks the surveillance and communications infrastructure to provide traditional traffic management services, especially as the density of drone operations increases over time.

% , due to the rapid growth of UAV  applications/ use cases, or In order
% Recreational UAVs that are used for digital photography are typically operated under visual line of sight (VLOS) conditions. However, with the increasing number of applications ranging from infrastructure inspection,  agriculture, transportation to assisting public safety agencies, the commercial UAVs tend to operate under BVLOS conditions.
% Given the number and type of UAV operations envisioned, it is identified that the existing Air Traffic Management (ATM) System infrastructure cannot scale cost-effectively 
% to support the exponential growth UAS.

% In order to truly unleash the potentials of UAVs, real-world and commercial deployments will most likely be in the form of beyond visual line-of-sight (BVLOS) scenarios, which in turn provide easier access to remote or hazardous areas, less human intervention, and reduced cost of operation~\cite{li2019beyond}. 
% % Yet, compared with the visual line-of-sight (VLOS) conditions, BVLOS carries higher safety risks. 



% However, the proliferation of new wireless services and the demand for higher cellular data rates have significantly exacerbated the spectrum crunch that cellular providers are already experiencing. Therefore, developing  dynamic spectrum management services to
% sense, assign, and monitor spectrum usage within the UTM architecture is of utmost importance in order to enable advanced UAV use cases in BVLOS, such as urban air mobility (UAM) and advanced air mobility (AAM)~\cite{rimjha2021urban}. 



% \subsection{Spectrum Needs for UAVs}
% \blue{[Need some more context here. Probably, adding one overall system model figure in the introduction and referring to that here, clarifies things. ]}

% As shown in Figure ~\ref{fig:scomp}, the methodology to compute spectrum requirements for a given coverage cell involves the information exchange between the UAVs, the spectrum efficiency, and the density of UAVs. To compute the total spectrum required we need to multiply the frequency reuse factor (K). 

% \begin{equation}
% W = K.B.M.R /(U.E)    
% \end{equation}
% where, K is the frequency reuse factor, B is the data rate requirement (kbit/s) for a single UAV, M is the UAV density in a single cell, U is the utlization factor ($\leq 1$), R is the redundancy factor ($\geq 1 $) that allow backup links, E is the spectral efficiency (bits/s/Hz). Finally, W (MHz)is the aggregate bandwidth requirement. Note that, the derivation of frequency reuse factor and different cell types are outlined in ~\cite{international2009characteristics,kakar2015uav}.

% In computing the requirements for both uplink (UL) and downlink (DL), we use the default values mentioned in ~\cite{international2009characteristics}. 
% Since we are computing the requirements for UAVs flying below 400 ft, we use cell type A for computing the estimated spectrum requirements for each cell. As seen in Figure ~\ref{fig:spec}, it can be clearly observed that as the UAV density (M) increases the total spectrum requirement increases. Note that the computations consider the UAV communications with video for command and control. 

% \blue{[This subsection on spectrum needs calculation is quite vague... Need more information.]}



% \begin{figure}[!htb]
% \minipage{0.48\textwidth}
%    \includegraphics[width=
%    \linewidth]{figures/spectrumcomputation.jpg}
%     % \caption{KPIs for UAV-assisted wireless services according to 3GPP TS 22.125, V17.1.0 }
%     % \label{fig:KPIWS}
%   % \includegraphics[width=\linewidth]{Figures/s.jpg}
%   \caption{ Methodology to compute spectrum requirements for each type of coverage cell as per ITU ~\cite{international2009characteristics}  }
%   \label{fig:scomp}
% \endminipage\hfill
% \vspace{2mm}
% \minipage{0.48\linewidth}
%   \includegraphics[width=\linewidth]{figures/specrequirementsUAV.jpg}
%   \caption{Estimated spectrum requirements for each type of coverage cell based on the guidelines defined in ~\cite{international2009characteristics}}
%   \label{fig:spec}
% \endminipage
% \end{figure}





% \begin{figure*}[!htb]
% \minipage{0.32\linewidth}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/spectrumcomputation.jpg}
%     \caption{ Methodology to compute spectrum requirements for each type of coverage cell as per ITU ~\cite{international2009characteristics} }
%     \label{fig:scomp}
%     \vspace{3mm}
%     \endminipage\hfill
% \end{figure*}
% \FloatBarrier

% \begin{figure*}[hbt!]
%     %\centering
%     \includegraphics[width=0.5\linewidth]{figures/specrequirementsUAV.jpg}
%     \caption{ Estimated spectrum requirements for each type of coverage cell based on the guidelines defined in ~\cite{international2009characteristics} }
%     \label{fig:spec}
%     \vspace{3mm}
% \end{figure*}


% \textbf{KPIs for UAV-assisted wireless services according to 3GPP }

% \blue{[What is the relation of this section with the previous? The paper needs to tell a story, and different parts should be connected. Right now, we have some unrelated paragraphs and sections.] }

% On the other hand, efforts are being made to include UAVs into the cellular network and several KPI's are defined in 3GPP Rel 17 and 18. As we can see in Figure~\ref{fig:KPIWS}, the UL and DL requirements for different UAV applications range from 300 Kbps to 100 Mbps. Few applications such as surveillance, delivery using line-of-sight links, video streaming, cellular-assisted UAV communication where an UAV can act as a base-station demand such data rates. Contrary to that, few studies ~\cite{wang2018bandwidth} has been conducted to evaluate the performance of UAV networks on LTE networks. It is concluded that 50 drones transmitting
% HD video streams continuously can saturate the theoretical
% uplink capacity of 500 Mbps in a 4G LTE cell that covers a large rural area. Moreover, if the transmission used 4k video streaming, the number of UAVs that can be supported in a cell further scales down ~\cite{abdalla2021communications}. It is clearly evident that UAVs with higher video resolution will saturate the 4G/5G network.

% As the demand for UAV applications increases, the UAV density increases. Hence, there would be a spectrum scarcity similar to the ground-based communications. In order to cope up with the existing spectrum demand and the anticipated new UAV applications, we have to consider dynamic spectrum sharing for UAVs. Few research exists on the theoretical aspects of the spectrum sharing for UAVs as discussed in section ~\ref{sec:relworks}

% \textbf{works on spectrum sensing}
% \textcolor{blue}{
% Authors in ~\cite{shang2020spectrum} investigate the need to design efficient spectrum sharing policies for UAV communications to enhance the spectral efficiency (SE) simultaneously controlling the interference-to-ground communications. Furthermore they propose spatial spectrum sensing (SSS) for UAV spectrum access and address several open research problems and challenges in applying SSS for UAV networks. While SSS was based on stochastic geometry and theoretical based several works proposed data driven spectrum sensing models. Authors in ~\cite{li2020deep,uvaydov2021deepsense}, proposed deep learning based spectrum sensing where spectrum holes are identified when primary users are not transmitting. However, the techniques did not consider dynamic UAV environments.
% }

% \textbf{works on sharing}
% \textcolor{blue}{
% Spectrum sharing is an active research area where the spectrum is shared among multiple technologies. Few studies focus assume the spectrum sensing results are available and built sharing models~\cite{sharing models without sensing}. Authors in ~\cite{cui2019multi} explore resource allocation strategies for UAVs based on multi agent reinforcement learning (MARL) framework. However, the UAVs are non co-operative and randomly select a channel to transmit.}

% However, the works so far didn't consider an integrated solution that detects the spectrum holes and allocates spectrum resources to the requesting UAVs. In this paper, we propose a coordinated spectrum sensing and sharing platform for UAVs.

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/KPI_WS.jpg}
%     \caption{KPIs for UAV-assisted wireless services according to 3GPP TS 22.125, V17.1.0 }
%     \label{fig:KPIWS}
%     \vspace{-3mm}
% \end{figure*}




==> results_old.tex <==
\vspace{-.2cm}
\section{Raw I/Q Dataset Generation}
\label{sec:dataset}
In the previous section, we described the role of DDQN in allocating spectrum holes to the SUs such that the overall utility is maximized. However, each SU has to first send in their spectrum hole detection results based on observed I/Q samples. 
% As we assume each UAV is capable of sensing $M$ sub-channels, implementing such wideband sensing techniques demand for efficient hardware and computing capabilities. 
Implementing a data-driven ML model for such wideband sensing demands large amounts of raw I/Q data. 
While it is desirable to capture over-the-air raw I/Q signals using actual hardware, it is challenging to accomplish this goal due to the intricate nature of flying multiple UAVs within a specific environment for collaborative sensing implementation.
Hence, we resort to generating synthetic dataset that accurately resembles collecting dataset via experimentation. 
% for different altitude and channel settings. However, to date the UAV based datasets are very limited and generating such datasets for our configuration is even more critical and pain-staking, hence we generate a synthetic dataset.
% The authors in~\cite{uvaydov2021deepsense} propose a method to generate synthetic LTE dataset using MATLAB. 
To this end, we use MATLAB's LTE toolbox as outlined in~\cite{uvaydov2021deepsense} and extend the dataset generation to incorporate UAV specifics. In particular, we generate the dataset by incorporating the LTE base-stations and UAVs locations, as well as 3D environment including buildings and vegetation for performing ray-tracing. 

% 

% Furthermore, they developed a wideband spectrum sensing method using the dataset generated and proposed an ML based multi-label classification for spectrum hole detection. The ML algorithm accepts raw I/Q samples and outputs the spectrum occupancy status.



%To generate such dataset, the channel occupancy has to be embedded into the dataset generation.




% light weight DL model for fast wideband sensing and a method for generating synthetic dataset using MATLAB. We take advantage of ML based multi-label classification setup to detect the spectrum holes as in ~\cite{uvaydov2021deepsense} and further extend to consider multiple UAVs and realistic LTE deployments.





% The authors in~\cite{uvaydov2021deepsense} propose a light weight DL model for fast wideband sensing and a method for generating synthetic dataset using MATLAB. We take advantage of ML based multi-label classification setup to detect the spectrum holes as in ~\cite{uvaydov2021deepsense} and further extend to consider multiple UAVs and realistic LTE deployments.

% The ML algorithm accepts raw I/Q samples and outputs the spectrum occupancy status. Since these operations are power hungry, we make the ML model as light as possible while still maintaining acceptable accuracy. Ideally we would like to capture over-the air raw I/Q signals from each UAV for different altitude and channel settings. However, to date the UAV based datasets are very limited and generating such datasets for our configuration is even more critical and pain-staking. To this reason, we generate a synthetic dataset using MATLAB's LTE toolbox. Furthermore, we generate the dataset as close to real world setting by incorporating the LTE base-station locations, 3D environment including building and vegetation for performing ray-tracing experiments.

\vspace{-1mm}
\begin{figure}[!htb]
\centering    \includegraphics[width=0.5\textwidth]{figures/datasetconfig_KC3_new.jpg}
    \vspace{-3mm}
    \caption{Simulation setup for dataset generation }    
    \label{fig:simsetup}
     \vspace{-4mm}
\end{figure}
\textbf{Dataset Generation Methodology.} As shown in Fig.~\ref{fig:simsetup}, we assume three neighboring cells.  In order to perform ray-tracing experiments, the maps required are downloaded from OpenStreetMap~\cite{OSM}.
% , a free and open geographic database updated and maintained by a community of volunteers via open collaboration~\cite{OSM}.

    %\vspace{-3mm}



The simulation area we considered is of $3$ km $\times$ $3$ km wide with buildings and vegetation. The location of the base stations are obtained from cellmapper~\cite{cellmap}, an open crowd sourced cellular tower and coverage mapping service. We define base-stations as the transmitter sites and UAV locations as the receiver sites. %The base station locations and UAV locations are given in Table~\ref{create table}.
%Also, we assume that UAV's are flying at an altitude of $90$ m. 
Furthermore, we consider three UAVs and three base stations in the region of interest, and use MATLAB's ray-tracer to find the channel between UAV and base-station locations. Note that this scenario can be easily extended to any numbers of LTE cells and UAVs. It is important to emphasize that we consider UAVs hovering in one location. Nevertheless, by executing the ray-tracing engine multiple times for different locations, we can effectively simulate a flight trajectory.

%}

% \begin{figure}[hbt!]
%     \includegraphics[width=0.35\textwidth]{figures/datasetconfig.jpg}
%     \caption{ Simulation setup for dataset generation  }
%     \label{fig:simsetup}
%     \vspace{-3mm}
% \end{figure}




% \begin{figure*}[!htb]
% \minipage{0.32\linewidth}
%   \includegraphics[width=\linewidth]{figures/Loc1.jpg}
%   \caption{Spectrum hole prediction Performance at UAV location 1 for varying SINR }\label{fig:loc1}
% \endminipage\hfill
% \minipage{0.32\linewidth}
%   \includegraphics[width=\linewidth]{figures/Loc2.jpg}
%   \caption{Spectrum hole prediction Performance at UAV location 2 for varying SINR}\label{fig:loc2}
% \endminipage\hfill
% \minipage{0.32\linewidth}%
%   \includegraphics[width=\linewidth]{figures/Loc3.jpg}
%   \caption{Spectrum hole prediction Performance at UAV location 3 for varying SINR}\label{fig:loc3}
% \endminipage
% \end{figure*}








% \newcommand{\var}[1]{\text{\texttt{#1}}}
% \newcommand{\func}[1]{\text{\textsl{#1}}}

% % \makeatletter
% \newcounter{phase}[algorithm]
% \newlength{\phaserulewidth}
% \newcommand{\setphaserulewidth}{\setlength{\phaserulewidth}}
% \newcommand{\phase}[1]{%
%   \vspace{-1.25ex}
%   % Top phase rule
%   \Statex\leavevmode\llap{\rule{\dimexpr\labelwidth+\labelsep}{\phaserulewidth}}\rule{\linewidth}{\phaserulewidth}
%   \Statex\strut\refstepcounter{phase}\textit{Phase~\thephase~--~#1}% Phase text
%   % Bottom phase rule
%   \vspace{-1.25ex}\Statex\leavevmode\llap{\rule{\dimexpr\labelwidth+\labelsep}{\phaserulewidth}}\rule{\linewidth}{\phaserulewidth}}
% \makeatother

% \setphaserulewidth{.7pt}

% \begin{algorithm}
%   \caption{Collaborative spectrum sensing and access for UAS in UTM systems}
%   \begin{algorithmic}[1]
%     \State initialization
%     \State $\var{ini} = 4$
%     \State $\var{init} = 0$
%     \phase{Spectrum Sensing }

%       \For{each UAV in~$\textbf{s}(t)\subseteq{\textbf{S}}$}
%         \State Capture I/Q samples from over the air signal
%         \State Broadcast IWD--
%         \For{each IWD}
%           \vspace{0.05in}
%           \State Compute $\func{soil}(i,j) = (1-\Pi\psi) \times \func{soil}(i,j)-\Pi\psi \Delta \func{soil}(i,j)$
%           \vspace{0.01in}
%           \State Compute $P_r = (i,j) = \frac{f(\func{soil}(i,j))}{\sum\nolimits_{k \notin \func{vc}(IWD)}{f(\func{soil}(i,k)}}$
%           \State $f(\func{soil}(i,j)) = \frac{1}{\func{soil}(i,j)}$
%         \EndFor
%       \EndFor


%     \phase{Broadcasting }
  
%     \For{each destination $D$ }
%     \State $\func{MPRset}(D) = \max\{P_r(z) \cup z \in R\}$
%     \State Send IWD-Rep $2$-hop away
%     \EndFor

%     \phase{Spectrum Fusion }

%       \For{each destination $D$ }
%         \State $\func{MPRset}(D) = \max\{P_r(z) \cup z \in R\}$
%         \State Send IWD-Rep $2$-hop away
%       \EndFor

%     \phase{Spectrum Access }

%       \For{each source $S$}
%         \State $\func{MPRset}(S) = \max\{P_r(z) \cup z \in R\}$ 
%       \EndFor
%       \State $\var{MPRRoute} = [S]$

%   \end{algorithmic}
% \end{algorithm}

% \noindent
% \textbf{Dataset description.} 
In the next step, we use MATLAB's LTE Toolbox to generate LTE-M waveform. The entire cell bandwidth of $10$ MHz ($50$ resource blocks) is assumed to be split into $16$ sub-channels each of size three resource blocks. In general, the base station can allocate a single sub-channel or multiple sub-channels to a PU to transfer user specific data on the downlink shared channel and also can use multiple access techniques for transmitting data to different PUs. However, when we generate the dataset we assume that base station partitions the bandwidth into separate sub-channels. While generating the downlink waveform of the base station we do not generate any UE specific reference  signals. Also, we do not corrupt the broadcast channels with user-specific data. We find the appropriate indices and embed the data samples into the downlink shared channel. As we assumed we partition the cell bandwidth into $16$ sub-channels, considering each combination as a label, the base station can generate $2^{16}$ labels, ranging from no sub-channel allocation to a fully busy cell site. 
% The DL is intended for primary users, however, as the base stations transmit with a higher output power, each SU receives the signal. 
Since we assumed all SUs are capable of wideband sensing, each SU samples the RF signal and stores I/Q samples. We vary the noise variance such that the effective SINR varies from $-10~\text{dB}$ to $20~\text{dB}$ in steps of $10~\text{dB}$. Here, the interference caters for the additional received signals from the neighboring base stations which are modeled using the ray-tracing setup as shown in Fig.~\ref{fig:simsetup}.

% For each location with a particular SINR, we generate approximately 200,000 samples. Hence we capture 2400,000 I/Q samples in total for all three UAV locations.  


% \newcommand{\var}[1]{\text{\texttt{#1}}}
% \newcommand{\func}[1]{\text{\textsl{#1}}}

% % \makeatletter
% \newcounter{phase}[algorithm]
% \newlength{\phaserulewidth}
% \newcommand{\setphaserulewidth}{\setlength{\phaserulewidth}}
% \newcommand{\phase}[1]{%
%   \vspace{-1.25ex}
%   % Top phase rule
%   \Statex\leavevmode\llap{\rule{\dimexpr\labelwidth+\labelsep}{\phaserulewidth}}\rule{\linewidth}{\phaserulewidth}
%   \Statex\strut\refstepcounter{phase}\textit{Phase~\thephase~--~#1}% Phase text
%   % Bottom phase rule
%   \vspace{-1.25ex}\Statex\leavevmode\llap{\rule{\dimexpr\labelwidth+\labelsep}{\phaserulewidth}}\rule{\linewidth}{\phaserulewidth}}
% \makeatother

% \setphaserulewidth{.7pt}

% \begin{algorithm}
%   \caption{Collaborative spectrum sensing and access for UAS in UTM systems}
%   \begin{algorithmic}[1]
%     \State initialization
%     \State $\var{ini} = 4$
%     \State $\var{init} = 0$
%     \phase{Spectrum Sensing }

%       \For{each UAV in~$\textbf{s}(t)\subseteq{\textbf{S}}$}
%         \State Capture I/Q samples from over the air signal
%         \State Broadcast IWD--
%         \For{each IWD}
%           \vspace{0.05in}
%           \State Compute $\func{soil}(i,j) = (1-\Pi\psi) \times \func{soil}(i,j)-\Pi\psi \Delta \func{soil}(i,j)$
%           \vspace{0.01in}
%           \State Compute $P_r = (i,j) = \frac{f(\func{soil}(i,j))}{\sum\nolimits_{k \notin \func{vc}(IWD)}{f(\func{soil}(i,k)}}$
%           \State $f(\func{soil}(i,j)) = \frac{1}{\func{soil}(i,j)}$
%         \EndFor
%       \EndFor


%     \phase{Broadcasting }
  
%     \For{each destination $D$ }
%     \State $\func{MPRset}(D) = \max\{P_r(z) \cup z \in R\}$
%     \State Send IWD-Rep $2$-hop away
%     \EndFor

%     \phase{Spectrum Fusion }

%       \For{each destination $D$ }
%         \State $\func{MPRset}(D) = \max\{P_r(z) \cup z \in R\}$
%         \State Send IWD-Rep $2$-hop away
%       \EndFor

%     \phase{Spectrum Access }

%       \For{each source $S$}
%         \State $\func{MPRset}(S) = \max\{P_r(z) \cup z \in R\}$ 
%       \EndFor
%       \State $\var{MPRRoute} = [S]$

%   \end{algorithmic}
% \end{algorithm}


\begin{figure}[!htb]
\minipage{0.48\linewidth}
\centering
  \includegraphics[width=\linewidth]{figures/precisionU3-new.png}
  \vspace{-7.5mm}
  \caption{\textbf{Precision} performance at location 3.}
  \label{fig:prec}
\endminipage\hfill
\minipage{0.48\linewidth}
\centering  \includegraphics[width=\linewidth]{figures/recallU3-new.png}
  \vspace{-7.5mm}
  \caption{\textbf{Recall} performance at location 3.}
  \label{fig:rec}
\endminipage\hfill
 \vspace{-6mm}
\end{figure}

\vspace{-.3cm}
\section{Numerical Results}
\label{sec:results}
\textbf{Collaborative Spectrum Sensing Results.}
As mentioned earlier, identifying spectrum holes falls into the realm of classical multi-class classification problem. We consider Precision, Recall, and F1-score as the metrics to assess the performance of such classifier. The general definitions of Precision and Recall are as follows: 

\vspace{-.2cm}
\small
\begin{equation}
     \text{Precision} = \frac{\text{TP}}{ \text{TP} + \text{FP}} ,\quad  \text{Recall} = \frac{\text{TP}}{ \text{TP} + \text{FN}},
\end{equation}   
% \begin{equation}
%      Recall = \frac{TP}{ TP + FN}
% \end{equation}
% \begin{equation}
%      F1-score = \frac{2(Precison . Recall)}{ Precison + Recall } ,
% \end{equation}
\normalsize
where TP, FN, FP accounts for the number of true positives, false negatives, and  false positives, respectively. 
% 
To concretely capture the performance of spectrum sensing across $16$ sub-channels, we compute the micro-averages for Precision and Recall~\cite{grandini2020metrics}.
% Note that F1-score metric can also be defined as the geometric mean of Precision and Recall. 
% While we can compute the metrics for each of the $16$ sub-channels, it would be ideal to have some sort of average performance. To this purpose, several averaging techniques like macro-averaging and micro-averaging exists in the literature~\cite{grandini2020metrics}. In this paper, we consider micro-averages for Precison, Recall and F1-score.
% In multi-label classification, when all the different labels have similar distribution, micro-average and macro-average would be identical. 

% The macro average and micro-average for precision are defined below:

% \small
% \vspace{-2mm}
% \begin{equation}
%      Precison(macro) = \frac{ \sum_{m=1}^{M} Precision(m)}{M},
% \end{equation}
% \begin{equation}
% Precison(micro) = \frac{ \sum_{m=1}^{M} TP(m)}{\sum_{m=1}^{M} TP(m) + FP(m)}.    
% \end{equation}
% \normalsize
% Similarly, we can define micro and macro averages for recall and F1-score can also be defined.

% \textbf{Spectrum sensing results obtained at different UAV location.} 
% We use $70\%$ of the samples generated to train the DNN while the rest of samples are used for testing and validation purpose. It can be observed in Fig.\ref{fig:loc1}, Fig.\ref{fig:loc2} and Fig.\ref{fig:loc3}, the performance metrics improve as the SINR improves. For UAV location1, and UAV location2, the performance metrics are greater than 90 $\% th$ percentile for SINR above $10dB$. For UAV location3, though the metrics improve as SINR improves, the received signal strength is weaker than the other two cases leading to more noise like I/Q samples. Hence, the ML model was not able to predict the spectrum holes as accurately as other UAV locations. This is one of the key observation for considering collaborative spectrum sensing in such dynamic environments. By combining the results of the SUs we can improve the reliability of overall spectrum sensing. %}



We use $70\%$ of the samples generated to train the DNN while the rest of samples are used for testing and validation purposes. We observed that the performance metrics improve as the SINR improves. Specifically, for UAV locations $1$ and $2$, the spectrum sensing performance metrics are greater than $90\%$ for the SINR values above $10~\text{dB}$. However, for UAV location 3, the overall performance metrics are worse than locations 1 and 2. As shown in Fig.~\ref{fig:prec} and \ref{fig:rec},  the performance metrics are about $90\%$ at $20~\text{dB}$ SINR. This is due to weaker received signal strength in location 3, leading to more noisy I/Q samples. Hence, the ML model was not able to predict the spectrum holes accurately, thereby making the rationale for exploring collaborative sensing more apparent.
% This is one of the key observation for considering collaborative spectrum sensing in such dynamic environments. 
% By combining the results of multiple UAVs we can improve the reliability and overall performance of spectrum sensing. 
From the spectrum fusion results (described in Eq.~\eqref{eqn:fusion}) shown in Fig.~\ref{fig:prec} and \ref{fig:rec}, we note that incorporating predictions from UAV locations 1 and 2 significantly 
% the performance metrics of UAV location $3$ improved 
improved the spectrum prediction performance. 
% Note that we considered majority rule as described in Eq.~\eqref{eqn:fusion}.%}



\textbf{Resource Allocation and Spectrum Access Results.}
As mentioned in Section~\ref{sec:problem2}, we use deep Q-learning methods for allocating spectrum resources to the UAVs. 
In Fig.~\ref{fig:dqn-1UAV}, we compare the training performance of three variants of Q-learning methods for allocating a sub-channel to a single UAV whenever the fusion rule detects at least a single spectrum hole. It is observed that DDQN with soft update performs slightly better and converges earlier than DDQN and vanilla-DQN. 
Next, we extend the model to allocate spectrum holes to two UAVs. In this case, we have augmented the DDQN algorithm with soft update to generate two best actions.  From the results in Fig.~\ref{fig:dqn-2UAV}, we observe that the utility performance with two SUs is slightly less than two times of the performance with a single SU. 
% proper tuning we can pick multiple best actions as shown in Fig.~\ref{fig:dqn-2UAV}. 
We further note that this paper tries to explore the possibility of integrating spectrum sensing and sharing by making use of existing RL algorithms. Though we explored Q-learning techniques, different RL algorithms can be integrated into the proposed framework.
% \vspace{-3mm}
% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.3\textwidth]{figures/dqn-1UAV-5k.png}
%     \vspace{-5mm}
%     \caption{Training results for allocating spectrum holes to \textbf{one UAV} using variations of deep Q-learning method. }
%     \label{fig:dqn-1UAV}
%      \vspace{-5mm}    
% \end{figure}





\begin{figure}[!t]
\minipage{0.48\linewidth}
\centering
 \includegraphics[width=\linewidth]{figures/dqn-1UAV-5k-new.png}
    \vspace{-8mm}
    \caption{Training results for allocating spectrum holes to \textbf{one UAV}.}
    % using variations of deep Q-learning method. }
    \label{fig:dqn-1UAV}
\endminipage
\vspace{-7mm}
\minipage{0.48\linewidth}
\centering
  \includegraphics[width=\linewidth]{figures/dqn-1-2UAV-5k-new.png}
     \vspace{-7mm}
    \caption{Training results for allocating spectrum holes to \textbf{two UAVs}.}
    \label{fig:dqn-2UAV}
\endminipage
% \vspace{-5mm}
\end{figure}

\vspace{-3mm}
% \begin{figure}[!htbp]
% \centering

    
%      \vspace{-5mm}    
% \end{figure}



% \vspace{-2mm}
% \begin{figure}[!htbp]
% \centering   
%      \vspace{-5mm}
   

% \subsection{Unified Collaborative Sensing and Access Results}
% \blue{[To be added]}
